Locking-free Simulation of Isometric Thin Plates

To efficiently simulate very thin, inextensible materials like cloth or paper, it is tempting to replace force-based thin-plate dynamics with hard isometry constraints. Unfortunately, naive formulations of the constraints induce membrane locking---artificial stiffening of bending modes due to the inability of discrete kinematics to reproduce exact isometries. We propose a simple set of meshless isometry constraints, based on moving-least-squares averaging of the strain tensor, which do not lock, and which can be easily incorporated into standard constrained Lagrangian dynamics integration.

==> 08_figs.tex <==
\section{Figures} \label{sec:figures}

\begin{figure*}[ht]
    \includegraphics[width=0.33\columnwidth,trim={8cm 0 0 0},clip]{figs/gravity.png}
    \includegraphics[width=0.33\columnwidth,trim={8cm 0 0 0},clip]{figs/gravity2.png}
    \includegraphics[width=0.33\columnwidth,trim={8cm 0 0 0},clip]{figs/gravity3.png}\\
    \includegraphics[width=0.33\columnwidth,height=0.1\textheight]{figs/gravity-2ring.png}
    \includegraphics[width=0.33\columnwidth,trim={8cm 0 0 0},clip]{figs/gravity-reg.png}
    \includegraphics[width=0.33\columnwidth,trim={8cm 0 0 0},clip]{figs/gravity-fine.png}\\
    \includegraphics[width=0.33\columnwidth,trim={8cm 0 0 0},clip]{figs/gravity-stiff.png}
    \includegraphics[width=0.33\columnwidth,trim={8cm 0 0 0},clip]{figs/gravity-soft.png}
    \includegraphics[width=0.33\columnwidth,trim={8cm 0 0 0},clip]{figs/gravity-softer.png}\\
    \includegraphics[width=0.33\columnwidth,trim={8cm 0 0 0},clip]{figs/gravity-goldenthal.png}
    \includegraphics[width=0.33\columnwidth,height=0.1\textheight]{figs/gravity-goldenthal2.png}
    \includegraphics[width=0.33\columnwidth,trim={8cm 0 0 0},clip]{figs/gravity-goldenthal3.png}
    \caption{Locking test on a square piece of cloth pinned at the corner. \emph{Top row}: simulation using our isometry constraints, from left to right: constraints tolerance 0.1, 0.01, and 0.001. Less sagging is observed as tolerance decreases. \emph{2nd row}: Our constraints on a regular mesh, finer irregular sampling, irregular sampling with twice the neighborhood size. All these simulations have similar curvature and do not lock. \emph{3rd row}: simulations using discrete elastic shells~\cite{Grinspun2006} for the same bending stiffness as our simulations, but varying stretching stiffnesses, decreasing from left to right. Notice there is no free lunch between excessive in-plane strain(sagging), and membrane locking. \emph{Bottom row}: simulation using edge length constraints ~\cite{Goldenthal} with same bending stiffness but varying diagonal spring stiffness decreasing from left to right. All results sag in the middle and fail to preserve isometry in this setup.}
    \label{fig:pinnedcloth}
\end{figure*}

\begin{figure}[ht]
\includegraphics[width=0.5\columnwidth]{figs/sphere-coarse.png}%
\includegraphics[width=0.5\columnwidth]{figs/sphere-fine.png}\\%
\includegraphics[width=0.5\columnwidth]{figs/box-coarse.png}%
\includegraphics[width=0.5\columnwidth]{figs/drapingBox.png}%
\caption{Draping experiments. Imposing our isometry constraints yields consistent results even for very coarse discretizations of the cloth (\emph{left column}). Despite the isometry constraints, cloth simulated by our method resolves the sharp edges of the box (\emph{bottom row}).}
\label{fig:draping}
\end{figure}

\begin{figure}[ht]
\includegraphics[width=0.5\columnwidth]{figs/temp-sphere-ours.PNG}%
\includegraphics[width=0.5\columnwidth]{figs/temp-sphere-lock.PNG}%
\caption{Locking experiments.Given the same bending stiffness, our method resolves the geometry of the underlying sphere(\emph{left}), while discrete shell method locks(\emph{right}).}
\label{fig:locking}
\end{figure}

\begin{figure}[ht]
\includegraphics[width=0.33\columnwidth]{figs/temp-tank.PNG}%
\includegraphics[width=0.33\columnwidth]{figs/temp-tank2.PNG}%
\includegraphics[width=0.33\columnwidth]{figs/temp-tank3.PNG}%
\caption{By changing bending stiffness(decreasing from left to right), our method simulates different materials without visible stretching.}
\label{fig:locking}
\end{figure}


